A Variational Dirichlet Framework for Out-of-Distribution Detection

With the recently rapid development in deep learning, deep neural networks have been widely adopted in many real-life applications. However, deep neural networks are also known to have very little control over its uncertainty for unseen examples, which potentially causes very harmful and annoying consequences in practical scenarios. In this paper, we are particularly interested in designing a higher-order uncertainty metric for deep neural networks and investigate its effectiveness under the out-of-distribution detection task proposed by~\cite{hendrycks2016baseline}. Our method first assumes there exists an underlying higher-order distribution $\mathbb{P}(z)$, which controls label-wise categorical distribution $\mathbb{P}(y)$ over classes on the K-dimension simplex, and then approximate such higher-order distribution via parameterized posterior function $p_{\theta}(z|x)$ under variational inference framework, finally we use the entropy of learned posterior distribution $p_{\theta}(z|x)$ as uncertainty measure to detect out-of-distribution examples. Further, we propose an auxiliary objective function to discriminate against synthesized adversarial examples to further increase the robustness of the proposed uncertainty measure. Through comprehensive experiments on various datasets, our proposed framework is demonstrated to consistently outperform competing algorithms.

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/dataset.tex <==
\begin{table*}[thb]
\small
\centering
\begin{tabular}{lllll} 
\toprule
Data Source                          & Dataset       & Content (classes)                                & \#Train & \#Test  \\ 
\midrule
\multirow{2}{*}{In-Distribution}     & CIFAR-10~\cite{krizhevsky2009learning}      & 10 classes: Airplane, Truck, Bird, etc.          & 60,000  & 10,000  \\
                                     & CIFAR-100~\cite{krizhevsky2009learning}     & 100 classes: Mammals,~ Fish, Flower, etc         & 60,000  & 10,000  \\ 
\midrule
\multirow{4}{*}{Out-of-Distribution} & iSUN~\cite{xiao2010sun}          & 908 clases: Airport, Abby, etc                   & -       & 8,925   \\
                                     & LSUN~\cite{yu2015lsun}          & 10 classes: Bedrooms, Churches, etc              & -       & 10,000  \\
                                     & Tiny-ImageNet~\cite{deng2009imagenet} & 1000 classes: Plant, Natural object, Sports, etc & -       & 10,000  \\
                                     & SVHN~\cite{netzer2011reading}          & 10 classes: The Street View House Numbers        & -       & 26,032  \\
\bottomrule
\end{tabular}
\caption{Overview of in- and out-of-distribution datasets}
\label{tab:dataset}
\end{table*}

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/table1.tex <==
% \usepackage{multirow}


\begin{table}
\small
\centering
\begin{tabular}{lllll} 
\hline
\begin{tabular}[c]{@{}l@{}}IND/OOD \\Model\end{tabular}                               & Method     & \begin{tabular}[c]{@{}l@{}}FPR\\@0.95\end{tabular} & \begin{tabular}[c]{@{}l@{}}Detection \\Error\end{tabular} & AUROC           \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\iSUN \\VGG13\end{tabular}}       & Baseline   & 43.8                                               & 11.4                                                      & 94              \\
                                                                                      & ODIN       & 22.4                                               & 10.2                                                      & 95.8            \\
                                                                                      & BNN        & 56.4                                               & 14.6                                                      & 91.2            \\
                                                                                      & Confidence & 16.3                                               & 8.5                                                       & 97.5            \\
                                                                                      & Ours       & \textbf{10.9}                                      & \textbf{6.9}                                              & \textbf{98.0}   \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\LSUN~\\VGG13\end{tabular}}       & Baseline   & 41.9                                               & 11.5                                                      & 94              \\
                                                                                      & ODIN       & 20.2                                               & 9.8                                                       & 95.9            \\
                                                                                      & BNN        & 52.4                                               & 14.2                                                      & 91.3            \\
                                                                                      & Confidence & 16.4                                               & 8.3                                                       & 97.5            \\
                                                                                      & Ours       & \textbf{9.9}                                       & \textbf{6.6}                                              & \textbf{98.1}   \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\TinyImgNet~\\VGG13\end{tabular}} & Baseline   & 43.8                                               & 12                                                        & 93.5            \\
                                                                                      & ODIN       & 24.3                                               & 11.3                                                      & 95.7            \\
                                                                                      & BNN        & 53.7                                               & 16.9                                                      & 90.2            \\
                                                                                      & Confidence & 18.4                                               & 9.4                                                       & 97              \\
                                                                                      & Ours       & \textbf{13.8}                                      & \textbf{7.9}                                              & \textbf{97.5}   \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SVHN/\\iSUN\\VGG13\end{tabular}}           & Baseline   & 10                                                 & 6                                                         & 98              \\
                                                                                      & ODIN       & 1.6                                                & 2.95                                                      & 99.5            \\
                                                                                      & Confidence & 0.9                                                & 2.3                                                       & 99.7            \\
                                                                                      & Ours       & \textbf{0.5}                                       & \textbf{1.8}                                              & \textbf{99.7}   \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SVHN/\\LSUN\\VGG13\end{tabular}}           & Baseline   & 9.4                                                & 5.7                                                       & 98.1            \\
                                                                                      & ODIN       & 1.4                                                & 2.6                                                       & 99.6            \\
                                                                                      & Confidence & 1                                                  & 2.3                                                       & 99.7            \\
                                                                                      & Ours       & \textbf{0.8}                                       & \textbf{2.2}                                              & \textbf{99.8}   \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SVHN/\\TinyImgNet\\VGG13\end{tabular}}     & Baseline   & 11.4                                               & 6.2                                                       & 97.8            \\
                                                                                      & ODIN       & 2.3                                                & 3.4                                                       & 99.3            \\
                                                                                      & Confidence & 1.5                                                & 2.8                                                       & 99.5            \\
                                                                                      & Ours       & \textbf{1.4}                                       & \textbf{2.3}                                              & \textbf{99.7}   \\
\hline
\end{tabular}
\caption{Experimental Results on VGG13 architecture, where Confidence refers to Learning Confidence algorithm~\cite{devries2018learning}, BNN refers to Bayesian Neural Network~\cite{gal2016uncertainty}.}
\label{tab:vgg}
\end{table}

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/table2a.tex <==
% \usepackage{multirow}


\begin{table}
\small
\centering
\begin{tabular}{lllll} 
\hline
IND/OOD     & \multirow{2}{*}{Method} & FPR            & Detection     & AUROC           \\
Dataset     &                         & @0.95          & Error         &                 \\ 
\hline
CIFAR-10/   & Baseline                & 52.6           & 13.6          & 92.4            \\
iSUN        & ODIN                    & 22.7           & 9.6           & 96.3            \\
ResNet18    & Semantic                & 21.5           & 9.2           & 96.3            \\
            & Ours                    & \textbf{13.8}  & \textbf{8.4}  & \textbf{97.1}   \\ 
\hline
CIFAR-10/   & Baseline                & 50.2           & 12.3          & 93.1            \\
LSUN        & ODIN                    & 17.9           & 8.4           & 96.9            \\
ResNet18    & Semantic                & 23             & 14            & 96              \\
            & Ours                    & \textbf{12.1}  & \textbf{6.3}  & \textbf{97.4}   \\ 
\hline
CIFAR-10/   & Baseline                & 59             & 15.1          & 91.1            \\
Tiny-ImgNet & ODIN                    & 32.1           & 11.2          & 94.9            \\
ResNet18    & Semantic                & 32.1           & 13.1          & 93.2            \\
            & Ours                    & \textbf{18.4}  & \textbf{9.9}  & \textbf{95.9}   \\ 
\hline
SVHN/       & Baseline                & 9.6            & 5.9           & 98              \\
iSUN        & ODIN                    & 1.1            & 2.7           & 99.6            \\
WideResNet  & Ours                    & \textbf{0.8}   & \textbf{1.8}  & \textbf{99.8}   \\ 
\hline
SVHN/       & Baseline                & 9.5            & 5.8           & 98              \\
LSUN-       & ODIN                    & 1.5            & 2.9           & 99.6            \\
WideResNet  & Ours                    & \textbf{0.6}   & \textbf{1.5}  & \textbf{99.8}   \\ 
\hline
SVHN/       & Baseline                & 10.6           & 6.1           & 97.8            \\
Tiny-ImgNet & ODIN                    & 2.1            & 3.2           & 99.5            \\
WideResNet  & Ours                    & \textbf{1.8}   & \textbf{2.8}  & \textbf{99.8}   \\
\hline
\end{tabular}
\caption{Experimental results for ResNet architecture, where Semantic refers to algorithm proposed in~\cite{shalev2018out}}
\label{tab:resnet}
\end{table}

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/table4.tex <==
% \usepackage{multirow}


\begin{table}
\small
\centering
\begin{tabular}{c|cccc} 
\hline
\multirow{2}{*}{Dataset} & \multicolumn{4}{c}{Cross-Entropy/Ours} \\
\cline{2-5}
                       & VGG13 & ResNet-18 & ResNet-34 & WideResNet\\
\hline
C-10                & 93.3/93.1  & 94.4/94.0       & -  & - \\
C-100               & -  &  -              & 79.4/79.1  & 80.5/80.7 \\ 
\hline
\end{tabular}
\caption{Classification accuracy of Dirichlet framework on CIFAR10/100 under different architectures.}
\label{tab:accuracy}
\end{table}

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/table_more_100.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table*}[thb]
\small
\centering
\begin{tabular}{lllccccc} 
\toprule
Model                                                                           & OOD & Method         & FPR@TPR95                 & Detection Error           & AUROC                     & AUPR~ In                  & AUPR Out                   \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}WideResNet\\CIFAR-100 \end{tabular}} & iSUN                                                   & Base/ODIN/Ours & 82.7/57.3/\textbf{18.0}  & 43.9/31.1/\textbf{11.1} & 72.8/86.6/\textbf{95.5} & 74.2/85.9/\textbf{95.5} & 69.2/84.9/\textbf{95.6}  \\
                                                                                & LSUN                                                   & Base/ODIN/Ours & 82.2/56.5/\textbf{13.3} & 43.6/30.8/\textbf{8.8}  & 73.9/86.0/\textbf{97.1} & 75.7/86.2/\textbf{97.1}  & 69.2/84.9/\textbf{97.2}  \\
                                                                                & TinyImgNet                                               & Base/ODIN/Ours & 79.2/55.9/\textbf{16.8} & 42.1/30.4/\textbf{10.2} & 72.2/84.0/\textbf{96.2}  & 70.4/82.8/\textbf{95.7} & 70.8/84.4/\textbf{96.4}   \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ResNeXt-29\\CIFAR-100 \end{tabular}} & iSUN                                                   & Base/ODIN/Ours & 82.2/61.6/\textbf{18.4}  & 31.0/21.4/\textbf{11.2} & 74.5/86.4/\textbf{94.9} & 79.8/89.1/\textbf{95.3} & 67.7/82.7/\textbf{94.0}   \\
                                                                                & LSUN                                                   & Base/ODIN/Ours & 82.2/62.4/\textbf{13.6}  & 31.8/22.1/\textbf{8.7}  & 73.6/85.9/\textbf{96.5} & 77.4/87.8/\textbf{96.8} & 69.5/83.9/\textbf{95.8}  \\
                                                                                & TinyImgNet                                               & Base/ODIN/Ours & 79.6/60.2/\textbf{16.9} & 31.0/21.5/\textbf{9.9}   & 75.1/86.5/\textbf{96.5} & 78.4/88.2/\textbf{96.8} & 71.6/84.8/\textbf{95.8}  \\
\bottomrule
\end{tabular}
\caption{More experimental results on CIFAR100 dataset on WideResNet and ResNeXt architeture.}
\label{tab:more_100}
\end{table*}

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/table_resnet_10.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[thb]
\small
\centering
\begin{tabular}{lllll} 
\midrule
\begin{tabular}[c]{@{}l@{}} IND/OOD\\Model \end{tabular}                                      & Method      & \begin{tabular}[c]{@{}l@{}} FPR@\\TPR95 \end{tabular} & \begin{tabular}[c]{@{}l@{}} Detection\\Error \end{tabular} & AUROC           \\ 
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}} CIFAR10/\\Tiny-ImgNet\\~\\ResNet18 \end{tabular}} & Baseline    & 59.0                                                  & 15.1                                                       & 91.1            \\
                                                                                              & ODIN        & 32.1                                                  & 11.2                                                       & 94.9            \\
                                                                                              & DPN         & 28.4                                                     & 13.6                                                          & 93.0            \\
                                                                                              & Mahalanobis & \textbf{2.9}                                          & \textbf{0.6}                                               & 96.3            \\
                                                                                              & Ours        & 17.1                                                  & 8.7                                                        & \textbf{96.8}   \\ 
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}} CIFAR10/\\LSUN\\~\\ResNet18 \end{tabular}}        & Baseline    & 50.2                                                  & 12.3                                                       & 93.1            \\
                                                                                              & ODIN        & 17.9                                                  & 8.4                                                        & 96.9            \\
                                                                                              & DPN         & 57.4                                                     & 20.5                                                          & 90.2            \\
                                                                                              & Mahalanobis & \textbf{1.2}                                          & \textbf{0.3}                                               & 97.5            \\
                                                                                              & Ours        & 7.7                                                   & 5.9                                                        & \textbf{98.3}   \\ 
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}} CIFAR10/\\SVHN\\~\\ResNet18 \end{tabular}}        & Baseline    & 49.5                                                  & 13.3                                                       & 92.0            \\
                                                                                              & ODIN        & 29.7                                                  & 15.1                                                       & 91.7            \\
                                                                                              & DPN         & 20.1                                                     & 12.7                                                          & \textbf{95.9}   \\
                                                                                              & Mahalanobis & \textbf{12.2}                                         & \textbf{2.3}                                               & 92.6            \\
                                                                                              & Ours        & 28.7                                                  & 13.6                                                       & 93.2            \\
\midrule
\end{tabular}
\caption{Experimental Results on ResNet18~\citep{he2016deep} architecture, where Mahalanobis refers to~\cite{lee2018simple} and DPN refers to~\cite{malinin2018predictive}, most results are copied from the original paper.}
\label{tab:resnet_10}
\end{table}

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/table_resnet_100.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[thb]
\small
\centering
\begin{tabular}{lllll} 
\toprule
\begin{tabular}[c]{@{}l@{}} IND/OOD\\Model \end{tabular}                                       & Method      & \begin{tabular}[c]{@{}l@{}} FPR@\\TPR95 \end{tabular} & \begin{tabular}[c]{@{}l@{}} Detection\\Error \end{tabular} & AUROC             \\ 
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} CIFAR-100/\\iSUN\\~\\ResNet34 \end{tabular}}       & ODIN        & 61.3                                                  & 23.7                                                       & 83.6              \\
                                                                                               & Semantic    & 58.4                                                  & 21.4                                                       & 85.2              \\
                                                                                               & Mahalanobis & \textbf{18.7}                                       & \textbf{11.6}                                            & 94.1              \\
                                                                                               & Ours        & 19.8                                                  & 12.2                                                       & \textbf{94.2}   \\ 
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} CIFAR-100/\\LSUN\\~\\ResNet34 \end{tabular}}       & ODIN        & 76.8                                                  & 42.4                                                       & 78.9              \\
                                                                                               & Semantic    & 79.5                                                  & 42.2                                                       & 79.0              \\
                                                                                               & Mahalanobis & 14.9                                                  & \textbf{9.0}                                             & 95.4              \\
                                                                                               & Ours        & \textbf{14.5}                                       & 9.6                                                        & \textbf{95.9}   \\ 
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR-100/\\Tiny-ImgNet\\~\\ResNet34 \end{tabular}} & ODIN        & 63.9                                                  & 25.2                                                       & 82.3              \\
                                                                                               & Semantic    & 62.4                                                  & 24.4                                                       & 83.1              \\
                                                                                               & Mahalanobis & \textbf{12.0}                                       & \textbf{9.1}                                             & \textbf{96.5}   \\
                                                                                               & Ours        & 16.3                                                  & 10.3                                                       & 95.3              \\
\bottomrule
\end{tabular}
\caption{Experimental results on ResNet34 architecture on CIFAR100 dataset, where Semantic refers to~\cite{shalev2018out} and Mahalanobis refers to~\cite{lee2018simple}.}
\label{tab:resnet_100}
\end{table}

==> [IJCAI19] A Variational Dirichlet Framework for Out-of-Distribution Detection/table_vgg.tex <==
% \usepackage{multirow}


\begin{table}[thb]
\small
\centering
\begin{tabular}{lllll} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}IND/OOD\\Model\end{tabular}}                     & \multirow{2}{*}{Method} & FPR@           & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Detection \\Error \end{tabular}} & \multirow{2}{*}{AUROC}  \\
                                                                                            &                         & TPR95          &                                                                             &                         \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\iSUN\\~\\VGG13\end{tabular}}           & Baseline                & 43.8           & 11.4                                                                        & 94                      \\
                                                                                            & ODIN                    & 22.4           & 10.2                                                                        & 95.8                    \\
                                                                                            & Confidence              & 16.3           & 8.5                                                                         & 97.5                    \\
                                                                                            & Semantic                & 23.2           & 10.2                                                                        & 96.4                    \\
                                                                                            & Ours                    & \textbf{10.7 } & \textbf{7.4 }                                                               & \textbf{97.7 }          \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\LSUN\\~\\VGG13\end{tabular}}           & Baseline                & 41.9           & 11.5                                                                        & 94                      \\
                                                                                            & ODIN                    & 20.2           & 9.8                                                                         & 95.9                    \\
                                                                                            & Confidence              & 16.4           & 8.3                                                                         & 97.5                    \\
                                                                                            & Semantic                & 22.9           & 13.9                                                                        & 96.0                    \\
                                                                                            & Ours                    & \textbf{10.3 } & \textbf{7.4 }                                                               & \textbf{97.8 }          \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\Tiny-ImgNet\\~\\VGG13\end{tabular}} & Baseline                & 43.8           & 12                                                                          & 93.5                    \\
                                                                                            & ODIN                    & 24.3           & 11.3                                                                        & 95.7                    \\
                                                                                            & Confidence              & 18.4           & 9.4                                                                         & 97                      \\
                                                                                            & Semantic                & 19.8           & 10.1                                                                        & 96.5                    \\
                                                                                            & Ours                    & \textbf{13.8 } & \textbf{7.9 }                                                               & \textbf{97.5 }          \\
\hline
\end{tabular}
\caption{Experimental Results on VGG13~\citep{simonyan2014very} architecture, where Confidence refers to~\cite{devries2018learning} and Semantic refers to~\cite{shalev2018out}, most results are copied from original paper.}
\label{tab:vgg}
\end{table}

==> table1.tex <==
% \usepackage{multirow}


\begin{table}
\small
\centering
\begin{tabular}{lllll} 
\hline
\begin{tabular}[c]{@{}l@{}}IND/OOD \\Model\end{tabular}                               & Method     & \begin{tabular}[c]{@{}l@{}}FPR\\@0.95\end{tabular} & \begin{tabular}[c]{@{}l@{}}Detection \\Error\end{tabular} & AUROC           \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\iSUN \\VGG13\end{tabular}}       & Baseline   & 43.8                                               & 11.4                                                      & 94              \\
                                                                                      & ODIN       & 22.4                                               & 10.2                                                      & 95.8            \\
                                                                                      & BNN        & 56.4                                               & 14.6                                                      & 91.2            \\
                                                                                      & Confidence & 16.3                                               & 8.5                                                       & 97.5            \\
                                                                                      & Ours       & \textbf{10.9}                                      & \textbf{6.9}                                              & \textbf{98.0}   \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\LSUN~\\VGG13\end{tabular}}       & Baseline   & 41.9                                               & 11.5                                                      & 94              \\
                                                                                      & ODIN       & 20.2                                               & 9.8                                                       & 95.9            \\
                                                                                      & BNN        & 52.4                                               & 14.2                                                      & 91.3            \\
                                                                                      & Confidence & 16.4                                               & 8.3                                                       & 97.5            \\
                                                                                      & Ours       & \textbf{9.9}                                       & \textbf{6.6}                                              & \textbf{98.1}   \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CIFAR10/\\TinyImgNet~\\VGG13\end{tabular}} & Baseline   & 43.8                                               & 12                                                        & 93.5            \\
                                                                                      & ODIN       & 24.3                                               & 11.3                                                      & 95.7            \\
                                                                                      & BNN        & 53.7                                               & 16.9                                                      & 90.2            \\
                                                                                      & Confidence & 18.4                                               & 9.4                                                       & 97              \\
                                                                                      & Ours       & \textbf{13.8}                                      & \textbf{7.9}                                              & \textbf{97.5}   \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SVHN/\\iSUN\\VGG13\end{tabular}}           & Baseline   & 10                                                 & 6                                                         & 98              \\
                                                                                      & ODIN       & 1.6                                                & 2.95                                                      & 99.5            \\
                                                                                      & Confidence & 0.9                                                & 2.3                                                       & 99.7            \\
                                                                                      & Ours       & \textbf{0.5}                                       & \textbf{1.8}                                              & \textbf{99.7}   \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SVHN/\\LSUN\\VGG13\end{tabular}}           & Baseline   & 9.4                                                & 5.7                                                       & 98.1            \\
                                                                                      & ODIN       & 1.4                                                & 2.6                                                       & 99.6            \\
                                                                                      & Confidence & 1                                                  & 2.3                                                       & 99.7            \\
                                                                                      & Ours       & \textbf{0.8}                                       & \textbf{2.2}                                              & \textbf{99.8}   \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SVHN/\\TinyImgNet\\VGG13\end{tabular}}     & Baseline   & 11.4                                               & 6.2                                                       & 97.8            \\
                                                                                      & ODIN       & 2.3                                                & 3.4                                                       & 99.3            \\
                                                                                      & Confidence & 1.5                                                & 2.8                                                       & 99.5            \\
                                                                                      & Ours       & \textbf{1.4}                                       & \textbf{2.3}                                              & \textbf{99.7}   \\
\hline
\end{tabular}
\caption{Experimental Results on VGG13 architecture, where Confidence refers to Learning Confidence algorithm~\cite{devries2018learning}, BNN refers to Bayesian Neural Network~\cite{gal2016uncertainty}.}
\label{tab:vgg}
\end{table}

==> table2a.tex <==
% \usepackage{multirow}


\begin{table}
\small
\centering
\begin{tabular}{lllll} 
\hline
IND/OOD     & \multirow{2}{*}{Method} & FPR            & Detection     & AUROC           \\
Dataset     &                         & @0.95          & Error         &                 \\ 
\hline
CIFAR-10/   & Baseline                & 52.6           & 13.6          & 92.4            \\
iSUN        & ODIN                    & 22.7           & 9.6           & 96.3            \\
ResNet18    & Semantic                & 21.5           & 9.2           & 96.3            \\
            & Ours                    & \textbf{13.8}  & \textbf{8.4}  & \textbf{97.1}   \\ 
\hline
CIFAR-10/   & Baseline                & 50.2           & 12.3          & 93.1            \\
LSUN        & ODIN                    & 17.9           & 8.4           & 96.9            \\
ResNet18    & Semantic                & 23             & 14            & 96              \\
            & Ours                    & \textbf{12.1}  & \textbf{6.3}  & \textbf{97.4}   \\ 
\hline
CIFAR-10/   & Baseline                & 59             & 15.1          & 91.1            \\
Tiny-ImgNet & ODIN                    & 32.1           & 11.2          & 94.9            \\
ResNet18    & Semantic                & 32.1           & 13.1          & 93.2            \\
            & Ours                    & \textbf{18.4}  & \textbf{9.9}  & \textbf{95.9}   \\ 
\hline
SVHN/       & Baseline                & 9.6            & 5.9           & 98              \\
iSUN        & ODIN                    & 1.1            & 2.7           & 99.6            \\
WideResNet  & Ours                    & \textbf{0.8}   & \textbf{1.8}  & \textbf{99.8}   \\ 
\hline
SVHN/       & Baseline                & 9.5            & 5.8           & 98              \\
LSUN-       & ODIN                    & 1.5            & 2.9           & 99.6            \\
WideResNet  & Ours                    & \textbf{0.6}   & \textbf{1.5}  & \textbf{99.8}   \\ 
\hline
SVHN/       & Baseline                & 10.6           & 6.1           & 97.8            \\
Tiny-ImgNet & ODIN                    & 2.1            & 3.2           & 99.5            \\
WideResNet  & Ours                    & \textbf{1.8}   & \textbf{2.8}  & \textbf{99.8}   \\
\hline
\end{tabular}
\caption{Experimental results for ResNet architecture, where Semantic refers to algorithm proposed in~\cite{shalev2018out}}
\label{tab:resnet}
\end{table}
